Sparse Binary Representation Learning for Knowledge Tracing

Knowledge tracing (KT) models aim to predict students' future performance based on their historical interactions. Most existing KT models rely exclusively on human-defined knowledge concepts (KCs) associated with exercises. As a result, the effectiveness of these models is highly dependent on the quality and completeness of the predefined KCs. Human errors in labeling and the cost of covering all potential underlying KCs can limit model performance. In this paper, we propose a KT model, Sparse Binary Representation KT (SBRKT), that generates new KC labels, referred to as auxiliary KCs, which can augment the predefined KCs to address the limitations of relying solely on human-defined KCs. These are learned through a binary vector representation, where each bit indicates the presence (one) or absence (zero) of an auxiliary KC. The resulting discrete representation allows these auxiliary KCs to be utilized in training any KT model that incorporates KCs. Unlike pre-trained dense embeddings, which are limited to models designed to accept such vectors, our discrete representations are compatible with both classical models, such as Bayesian Knowledge Tracing (BKT), and modern deep learning approaches. To generate this discrete representation, SBRKT employs a binarization method that learns a sparse representation, fully trainable via stochastic gradient descent. Additionally, SBRKT incorporates a recurrent neural network (RNN) to capture temporal dynamics and predict future student responses by effectively combining the auxiliary and predefined KCs. Experimental results demonstrate that SBRKT outperforms the tested baselines on several datasets and achieves competitive performance on others. Furthermore, incorporating the learned auxiliary KCs consistently enhances the performance of BKT across all tested datasets.

==> sections/down_stream.tex <==
\section{Application of Learned Latent Knowledge Components in Downstream Tasks}

The binary multi-hot vectors representing latent knowledge components (KCs), denoted as $\mathbf{u}_{\text{Ex}}$, not only enhance the predictive capabilities of our model but also serve as valuable features for downstream tasks. In this section, we discuss how these learned latent KCs can be utilized in other models to improve performance and examine whether they constitute disentangled representations.

\subsection{Utilizing Latent KCs in Downstream Models}

The binary vectors $\mathbf{u}_{\text{Ex}} \in \{0, 1\}^M$, obtained from the quantization algorithm applied to exercise embeddings, encapsulate the latent KCs associated with each exercise. These vectors can be extracted from our model and used as input features for various downstream tasks, such as:

\begin{itemize}
    \item \textbf{Student Modeling:} Enhancing models that predict student performance by providing a more granular understanding of the knowledge components involved in exercises.
    \item \textbf{Curriculum Design:} Informing the creation of learning paths by identifying which latent KCs are most critical for mastering certain concepts.
    \item \textbf{Exercise Recommendation:} Improving recommendation systems by matching exercises to students based on the latent KCs they have or have not mastered.
\end{itemize}

By incorporating $\mathbf{u}_{\text{Ex}}$ into these models, we leverage the rich, learned representations that capture underlying patterns in the data, leading to improved performance compared to using raw exercise embeddings or traditional KC labels alone.

\subsection{Benefits of the Learned Latent KCs}

The advantages of using the learned latent KCs in downstream tasks include:

\begin{itemize}
    \item \textbf{Improved Interpretability:} The binary nature of $\mathbf{u}_{\text{Ex}}$ simplifies interpretation, as each dimension corresponds to the presence or absence of a specific latent KC.
    \item \textbf{Dimensionality Reduction:} Compared to high-dimensional embeddings, the binary vectors provide a more compact representation, reducing computational complexity.
    \item \textbf{Enhanced Performance:} Empirical results demonstrate that models incorporating $\mathbf{u}_{\text{Ex}}$ achieve better performance due to the informative and discriminative nature of the latent KCs.
\end{itemize}

\subsection{Disentanglement of Latent Representations}

The concept of \emph{disentangled representations} refers to feature representations where individual dimensions capture distinct, interpretable factors of variation in the data. In our context, the binary vectors $\mathbf{u}_{\text{Ex}}$ can be considered as disentangled representations for the following reasons:

\begin{enumerate}
    \item \textbf{Distinct Latent KCs:} Each dimension in $\mathbf{u}_{\text{Ex}}$ corresponds to a specific latent KC, representing a unique aspect of the exercise that contributes to student learning.
    \item \textbf{Independent Factors:} The quantization algorithm promotes sparsity by selecting the top-$C_{\text{max}}$ components, encouraging the model to capture independent factors rather than entangled features.
    \item \textbf{Interpretability:} The binary values (0 or 1) indicate the absence or presence of a latent KC in an exercise, making the representation easily interpretable and facilitating analysis in downstream tasks.
\end{enumerate}

By producing disentangled representations, our model aids in uncovering the underlying structure of educational data. This disentanglement is beneficial for tasks that require an understanding of the specific knowledge components involved in learning processes.

\subsection{Implications for Educational Data Mining}

The ability to extract and utilize disentangled latent KCs has significant implications for educational data mining:

\begin{itemize}
    \item \textbf{Personalized Learning:} Educators and adaptive learning systems can tailor instruction based on the specific latent KCs a student struggles with or has mastered.
    \item \textbf{Knowledge Discovery:} Researchers can analyze the latent KCs to uncover hidden patterns and relationships between different concepts and exercises.
    \item \textbf{Model Generalization:} Models using disentangled representations may generalize better to new data, as they capture fundamental aspects of the learning process.
\end{itemize}



==> sections/subsections/binary.tex <==

\section*{Quantization Algorithm for Generating Binary Multi-Hot Vectors}

The quantization algorithm maps the output of the single-layer MLP (\( \mathbf{h} \)) to a binary (multi-hot) vector \( \mathbf{u}_q \) that encodes the latent knowledge components (KCs) associated with a given exercise. This algorithm allows flexibility in the number of active KCs per exercise, up to a specified maximum \( c_{\text{max}} \). The algorithm operates as follows:

\subsection*{Inputs:}
\begin{itemize}
    \item \( \mathbf{h} \in \mathbb{R}^m \): The output of the single-layer MLP for an exercise, where \( m \) is the dimensionality of the latent space.
    \item \( c_{\text{max}} \in \mathbb{N} \): The maximum number of active latent KCs (non-zero entries) allowed in the resulting multi-hot vector.
\end{itemize}

\subsection*{Algorithm:}

1. \textbf{Top-\( c_{\text{max}} \) Selection:} Identify the indices of the top \( c_{\text{max}} \) largest values in \( \mathbf{h} \) (by magnitude), denoted as \( \mathcal{I}_{\text{top}} \subseteq \{1, 2, \dots, m\} \). Create a mask \( \mathbf{m} \in \{0, 1\}^m \) where:
   \[
   \mathbf{m}[i] =
   \begin{cases}
   1, & \text{if } i \in \mathcal{I}_{\text{top}}, \\
   0, & \text{otherwise}.
   \end{cases}
   \]
   This mask serves as the initial binary indicator for the active dimensions.

2. \textbf{Binary Transformation:} To introduce flexibility in encoding, apply the following transformation to \( \mathbf{h} \):
   \[
   \mathbf{b} = \frac{\operatorname{sign}(\mathbf{h}) + 1}{2},
   \]
   where \( \operatorname{sign}(x) \) returns:
   \[
   \operatorname{sign}(x) =
   \begin{cases}
   1, & x > 0, \\
   0, & x = 0, \\
   -1, & x < 0.
   \end{cases}
   \]
   This transformation maps \( \mathbf{h} \) to values in \( \{0, 0.5, 1\} \). Any resulting \( 0.5 \) values are treated as \( 1 \) during downstream tasks.

3. \textbf{Mask Application:} Combine the mask \( \mathbf{m} \) and the binary-transformed vector \( \mathbf{b} \) to generate the final multi-hot vector \( \mathbf{u}_q \in \{0, 1\}^m \):
   \[
   \mathbf{u}_q[i] = \mathbf{m}[i] \cdot \mathbf{b}[i].
   \]

\subsection*{Training with Gradient Descent:}

To enable training of this discrete mapping using stochastic gradient descent, the \textbf{straight-through estimator (STE)} is applied. The STE treats the binary activation function as follows:
\begin{itemize}
    \item \textbf{Forward Pass:} The binary activation function is treated as the identity function, allowing the network to compute \( \mathbf{u}_q \) directly.
    \item \textbf{Backward Pass:} The binary activation function is treated as the identity function for gradient computation, i.e., the gradient is passed through as if the function were continuous:
    \[
    \frac{\partial \mathbf{u}_q}{\partial \mathbf{h}} = \mathbf{1}.
    \]
    This avoids gradient flow through the discrete thresholding operations, allowing the network to update the parameters of the MLP smoothly.
\end{itemize}



==> sections/subsections/model_prediction.tex <==

\section*{Prediction Model}

Building on the representations described earlier, the model predicts the probability of a correct response for future student interactions by integrating the multi-hot vectors \( \mathbf{v}_{\text{KC}} \) (for KCs) and \( \mathbf{v}_{\text{Q}} \) (for latent KCs derived from exercise embeddings). These representations are used as follows:

\subsection*{Unified Representation}

The labeled multi-hot vectors \( \mathbf{v}_{\text{KC}} \in \{0, 1\}^{2n} \) and \( \mathbf{v}_{\text{Q}} \in \{0, 1\}^{2m} \), described previously, are concatenated to form a unified feature vector:
\[
\mathbf{v}_{\text{total},t} = [\mathbf{v}_{\text{KC},t} \; \oplus \; \mathbf{v}_{\text{Q},t}] \in \{0, 1\}^{2n + 2m}.
\]
This vector combines information about both the KCs and the latent KCs, including their correctness labels.

\subsection*{Dimensionality Reduction}

The concatenated vector \( \mathbf{v}_{\text{total},t} \) is mapped to a dense representation suitable for sequence modeling through a linear transformation:
\[
\mathbf{v}_{\text{RNN-ready},t} = \mathbf{M} \mathbf{v}_{\text{total},t},
\]
where \( \mathbf{M} \in \mathbb{R}^{d \times (2n + 2m)} \) is a trainable weight matrix, and \( \mathbf{v}_{\text{RNN-ready},t} \in \mathbb{R}^d \) is the reduced feature vector.

\subsection*{Sequence Modeling}

The sequence of feature vectors \( \{\mathbf{v}_{\text{RNN-ready},1}, \mathbf{v}_{\text{RNN-ready},2}, \dots, \mathbf{v}_{\text{RNN-ready},T}\} \), corresponding to a student’s interactions over time, is fed into a recurrent neural network (RNN). The RNN models the temporal dynamics of the interactions, with the hidden state \( \mathbf{h}_t \in \mathbb{R}^h \) at each time step computed as:
\[
\mathbf{h}_t = \text{RNN}(\mathbf{v}_{\text{RNN-ready},t}, \mathbf{h}_{t-1}),
\]
where \( h \) is the dimensionality of the RNN’s hidden state.

\subsection*{Prediction}

The RNN hidden state \( \mathbf{h}_t \) is passed through a single-layer multi-layer perceptron (MLP) to produce logits for the relevance of each KC and latent KC:
\[
\mathbf{o}_t = \mathbf{W}_{\text{out}} \mathbf{h}_t + \mathbf{b}_{\text{out}},
\]
where \( \mathbf{W}_{\text{out}} \in \mathbb{R}^{(n + m) \times h} \) and \( \mathbf{b}_{\text{out}} \in \mathbb{R}^{n + m} \) are trainable parameters, and \( \mathbf{o}_t \in \mathbb{R}^{n + m} \) is the output vector.

To compute the final prediction, the binary multi-hot vectors \( \mathbf{u}_{\text{KC}} \in \{0, 1\}^n \) and \( \mathbf{u}_{\text{Q}} \in \{0, 1\}^m \), described earlier, are concatenated:
\[
\mathbf{u}_{\text{total},t} = [\mathbf{u}_{\text{KC},t} \; \oplus \; \mathbf{u}_{\text{Q},t}].
\]
The predicted probability of a correct response is then obtained by taking the dot product of \( \mathbf{u}_{\text{total},t} \) with \( \mathbf{o}_t \), followed by applying the sigmoid activation function:
\[
\hat{y}_t = \sigma(\mathbf{u}_{\text{total},t}^\top \mathbf{o}_t),
\]
where \( \sigma(\cdot) \) denotes the sigmoid function.


